M$^3$Exam: Benchmarking Multimodal Memory for Realistic User-Agent Interactions

Language agents are increasingly deployed over accumulating multimodal information, yet existing benchmarks assume a human-human form with sparse visuals and straightforward content, evaluating neither reasoning over authentic multimodal file interaction nor the interpretation of concealed user information. We therefore introduce M$^3$Exam, a query-centric multimodal conversational memory benchmark built on realistic user-agent interaction, with multi-dimensional evaluation spanning cross-modal grounding and implicit information inference. Benchmarking MLLMs and memory systems reveals persistent gaps in cross-modal grounding, cross session reasoning, and the efficiency cost of accumulating multimodal context. We further propose M$^3$Proctor, a multimodal memory method that detects query modality bias and consumes raw visual sources only on demand, improving accuracy by 13% while cutting index-construction time and retrieved tokens by over 70%.

==> sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/Teaser.pdf}
  \caption{Overview of \benchmark.}
  \label{fig:overview}
\end{figure}

Multimodal large language models (MLLMs) have advanced rapidly from 
single-turn visual question answering toward serving as 
general-purpose conversational agents in users' daily 
workflows~\cite{qwen2025vl,liu2024llavanext,gemini2024_15}, expanding their role 
to serving as persistent personal agents that organize 
and reason over heterogeneous multimodal artifacts~\cite{cheng2025higher}. 
This shift transforms the central challenge from per-turn 
perception to managing long-term multimodal histories, demanding 
more durable and well-structured memory.
While a growing line of work augments agents 
with external memory structures~\cite{zhang2025survey}, their support for 
cross-modal retrieval and reasoning remains systematically 
under-evaluated.

\begin{table*}[t]
\centering
\small
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\centering\arraybackslash}p{5.0cm}}
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{0.95}
\begin{tabularx}{\linewidth}{L|YY|YYYY|YY}
\toprule
\multirow{2}{*}{\centering\textbf{Benchmark}}
 & \multicolumn{2}{c|}{\textbf{Memorizing}}
 & \multicolumn{4}{c|}{\textbf{Reasoning}}
 & \multicolumn{2}{c}{\textbf{Interpreting}} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-7}\cmidrule(lr){8-9}
 & \textbf{A.\,Round} & \textbf{A.\,File}
 & \textbf{CM} & \textbf{CMQA} & \textbf{FM} & \textbf{SA}
 & \textbf{II} & \textbf{TH} \\
\midrule
LongMemEval~\citep{wu2025longmemeval}     & 5.2  & --   & \No   & \No   & \No   & \No & \No & \No   \\
MemoryArena~\citep{he2026memoryarena}     & 6.9  & --   & \No   & \No   & \No   & \No & \No  & \No   \\
MemoryAgentBench~\citep{hu2025evaluating} & 9.6  & --   & \No   & \No   & \No   & \No & \Part & \Part   \\
LoCoMo~\citep{maharana2024locomo}         & 10.8 & 3.4  & \Part & \Part & \No   & \No & \No & \No   \\
MMDialog~\citep{feng2023mmdialog}         & 4.6  & 2.6  & \Part & \Part & \Part & \No & \No   & \No   \\
MMRC~\citep{xue2025mmrc}                  & 12.9 & 2.9  & \Yes  & \Yes  & \Yes  & \No & \No   & \No   \\
Mem-Gallery~\citep{bei2026mem}            & 16.5 & 4.2  & \Yes  & \Yes  & \Yes  & \No & \No & \No \\
\midrule
\rowcolor{skyblue}
\textbf{\benchmark (Ours)}
 & \textbf{12.7} & \textbf{7.5}
 & \Yes & \Yes & \Yes & \Yes
 & \Yes & \Yes \\
\bottomrule
\end{tabularx}
\caption{Comparison of \benchmark with representative
conversational-memory benchmarks.
% across three capability families
\textbf{A.\,Round} = average user--assistant
rounds per session; \textbf{A.\,File} = average images and document
files per session.
\textbf{CM} = cross-modal retrieval;
\textbf{CMQA} = cross-modal QA requiring fusion of visual and
textual evidence; \textbf{FM} = file management and retrieval;
\textbf{SA} = statistical analysis of multimodal graphs.
\textbf{II} = implicit information inference;
\textbf{TH} = thematic domain-specific thematic reasoning.
\Yes{} = supported; \Part{} = partial / restricted; \No{} = not
supported; -- = N/A.}
\label{tab:bench-compare}
\end{table*}

Based on these observations, we argue that a comprehensive 
multimodal memory benchmark should mirror how humans engage with 
information: we must first \emph{memorize} what we encounter, 
\emph{reason} over it to connect disparate pieces, and \emph{interpret} 
concealed information beyond its literal phrasing. These three modes of engagement motivate three corresponding 
dimensions of complexity. \emph{1. Content Complexity}: heterogeneous 
artifacts spanning dialogue, images, and document files such as 
PDFs accumulated across sessions, \emph{2. Reasoning Complexity} 
: cross-modal grounding and multi-step inference over stored 
content, and \emph{3. Interpret Complexity}: queries whose answers hinge on
unstated, user-specific cues rather than literal surface content.

% \textcolor{red}{we must first \emph{memorize} what we encounter, 
% \emph{retrieve} over it to connect disparate pieces, and \emph{reason} 
% concealed information beyond its literal phrasing. These three modes of engagement motivate three corresponding 
% dimensions of complexity. \textbf{1. Content Complexity}: heterogeneous 
% artifacts accumulated across sessions, spanning dialogue, images, and 
% document files such as PDFs. \textbf{2. Retrieval Complexity}: relevant evidence is often fragmented 
% across sessions, modalities, and knowledge sources, making it difficult 
% to identify and recall. 
% \textbf{3. Reasoning Complexity}: answering requires grounding and 
% multi-step inference over the retrieved evidence beyond surface-form 
% matching.}

Existing benchmarks fall short on all three fronts. Long-term
conversational memory suites are text-only and omit visual modalities
\cite{wu2024longmemeval,he2026memoryarena}, while multimodal
counterparts treat images as incidental snapshots and ignore
document-level artifacts \cite{maharana2024locomo,bei2026mem}.
% 这里我大概理解是想表达agent memory里面没有document，document里面没有agent memory。
% 但感觉这里单独提出来一个document QA有点怪，有点太具体了，因为还有visual-QA啥的，看能不能咋圆一下，或者就不提别的类型的benchmark了，就强调agent memory的benchmark
% 这里讲limitation的时候和前面的complexity对上，现在相当于对应了第一个complexity，还差第二个complexity，感觉可以在讲完复杂模态之后放在一起说了，后面那个intent算是对应了第三个complexity。
\textcolor{red}{Document QA benchmarks} probe rich multimodal reasoning but confine it
to a single file in a single turn
\cite{tanaka2023slidevqa,ma2024mmlongbench}. 
% 这里要改一下，这个current query不足和prior context两个说法很容易让人误解成multi-turn多轮对话那种存在指代关系之类的，多个query之间有逻辑关系的情况；根据数据集情况具体把这句话要表达的内容改一下
\textcolor{red}{Crucially, nearly all
assume user intent is fully expressed in the current query, sidestepping
the \emph{implicit-intent} regime where answers depend on domain
knowledge or prior context the user never restates.}
To address these limitations, we introduce \benchmark, 
% 这里突然提出query centric这个词有点突兀，最好是上下文逻辑有联系：比如说上面你说数据集里面最重要的应该是以query为中心的xxxxx，which 解释是xxxx。后面再说提出来query centric。
% 现在上面强调的是 implicit-intent，那这里benchamrk也最好强调的是 implicit-intent，或者加一句解释，解释query centric和implicit-intent之间的逻辑关系，比如后面加一句which 以解析query中的xxxx，构造implicit intent xxxx，形成的benchmark。
% 大概这种意思
a
\textcolor{red}{query-centric} multimodal conversational QA benchmark spanning analytic, narrative, and document-grounded domains.
It comprises 239 multi-session conversations ($3{,}025$ rounds,
$1{,}799$ images and files) and $5{,}150$ evaluation
items, of which \textbf{1{,}975} are cross-modal items unanswerable
from text alone. Beyond standard recall and multi-hop questions,
\benchmark adds two types absent from prior benchmarks:
\textbf{Thematic Reasoning (TH)}, requiring domain knowledge implicit
in the user's context, and \textbf{Implicit Inference (II)}, where the
answer hinges on unstated intent that must be inferred from accumulated
evidence.

We further turn our findings into a method. Our analysis shows that
existing multimodal memory systems are \emph{modality-agnostic}: they
index and re-feed raw visual sources indiscriminately, so the per-query
token budget is dominated by image tokens spent on questions a textual
surrogate could already answer. 
% 前面强调的点是multi modal 和 intent啥的，这里只说了multi modal，然后又从效率方面说提高了，没说怎么解决**前面提到过的多模态记忆的难点**和**前面提到过的query-intent啥的**，感觉有点对不上。
\textcolor{red}{We therefore propose \method, a
modality-aware cascade that reads the \emph{modality bias} of a query
and prefers the cheapest representation that still answers it}, via
(1) cached modality-bias detection, (2) bias-aware re-ranking over dense
retrieval, and (3) cost-aware cascaded answering that escalates to raw
visual sources only when a confidence test fails. Compared to proposed multimodel memory systems,
\method improves accuracy by over 13.8\% with 70\% less tokens
while cutting index-construction time by over 80\%. Overall, our main contributions are summarized as follows:
\begin{itemize}
\item We construct \benchmark, a multimodal conversational
QA benchmark spanning 15 persona scenarios of 239 multi-session
conversations with rich cross-modality reasoning and intention interpretaion evaluations.
\item We conduct extensive benchmarking and in-depth analyses across
open MLLMs and multimodal memory systems, systematically uncovering their limitations
in incremental visual grounding and the efficiency problem of accumulating multimodal context.
\item We propose \method, a modality-aware retrieval method that detects
query modality bias and enables modality cascade to consume raw visual sources only on demand. On
\benchmark, \method improves accuracy by 13.8\% with significantly less cost.
\end{itemize}

==> sections/03_datasetintro.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/Main_Graph.pdf}
  \caption{Overall pipeline of \benchmark, designed to evaluate multimodal memory ability in realistic scenarios.}
  \label{fig:overview}
\end{figure*}


\section{\benchmark: Towards Realsitic Benchmark}
\label{sec:benchmark}

This section introduces \benchmark in detail (Figure~\ref{fig:overview}).§

\subsection{Task Formulation}
\label{sec:taskdefine}
\rmark{ModalityTalk casts the agent as a respondent over an accumulating multimodal memory. Each instance pairs a multi-session conversation $\mathcal{D}$ with a query $x$ forming a history $\mathcal{H}$ ... the agent must produce an answer $\hat{a}=f(x,\mathcal{H})$, scored against the gold $a_0$ ... Each query is annotated with the set $\mathcal{F}_q$ of supporting-fact rounds it depends on ... so answering requires retrieving the right evidence from $\mathcal{H}$, grounding across text/images/documents, and interpreting unstated intent. A memory-augmented agent additionally indexes $\mathcal{H}$ and retrieves $\mathcal{R}\subseteq\mathcal{H}$ ... so $\hat{a}=f(x,\mathcal{R})$; the benchmark then evaluates both the answer and how well $\mathcal{R}$ covers $\mathcal{F}_q$.}

% =====================================================================
\subsection{Source Inputs}
\label{sec:src-inputs}

% 图片里面提到了 Factual Anchoring，可以把这个词放在这里说一下，一般人都是先看图再在内容里找介绍。
\textcolor{red}{The data generation pipeline is parameterized by three inputs.}
\textbf{(1) A user persona} $\mathcal{P}$ is a short biographical
description (name, profession, interests, characteristics) that
grounds and steers event generation.
\textbf{(2) A core event} $\mathcal{C}$ is a one-paragraph narrative
arc that the persona pursues over time and that all on-topic events
must advance. \textbf{(3) Multimodal file pool} $\mathcal{F}$ supplies the visual
evidence---charts, photographs, or PDF documents, provided locally or
later retrieved by keyword---and is persona-aligned so attached
artifacts are plausible for the persona. The pipeline maps the triple
$(\mathcal{P}, \mathcal{C}, \mathcal{F})$ to a benchmark in which every
event, dialogue turn, and question is anchored to these inputs.
Swapping the triple instantiates a new domain with no change to the
pipeline, while the alignment constraints keep the output faithful to
the specification.

% =====================================================================
\subsection{Timeline Generation}
\label{sec:timeline}

\noindent \textbf{Core-event line.}
Conditioned on $(\mathcal{P}, \mathcal{C})$, a text LLM generates a
chronologically ordered \emph{core-event line} of $N$ events
$\{e_1, \dots, e_N\}$. Each event $e_i$ is a structured record as follows:
\begin{equation}
  e_i = (\textsc{idx}_i,\ \textsc{desc}_i,\ \textsc{query}_i,\
         \textsc{time}_i,\ \textsc{kw}_i),
\end{equation}
where $\textsc{desc}_i$ describes what happens in the persona's life,
$\textsc{query}_i$ is the \emph{event-arised query} the persona will
raise (sharing visuals and asking a specific question),
$\textsc{time}_i$ is an absolute date that strictly increases with
$i$, and $\textsc{kw}_i$ is a short keyword used to retrieve the
event's images.

\noindent \textbf{Distractor side events.}
Real users do not stay perfectly on-topic. To inject realistic noise,
we generate $M$ distractor side events from domains
orthogonal to $\mathcal{C}$ (everyday errands, hobbies, casual
chatter, etc.). These events follow the same record schema but are flagged
$\textsc{distract}{=}\texttt{true}$, and are merged into the core line
by date and renumbered, yielding the final timeline.
By interleaving these off-topic events, distractors test whether a model
can locate the key relevant evidence without being misled by surrounding noise.

% \noindent \textbf{Quality Control.} The timeline is first validated by an LLM \emph{self-check} that audits three failure modes: persona violations (wrong name, profession, or
% behavior inconsistent with $\mathcal{P}$), core-event violations
% (on-topic events that fail to advance or in collision with $\mathcal{C}$), 
% and internal contradictions (date-order or mutually
% exclusive states). Guided by this audit report, an expert performs a final spot-check on
% persona consistency and core-event coverage before the timeline enters
% synthesis.

% =====================================================================
\subsection{Conversation Synthesis}
\label{sec:conv-synthesis}

\noindent \textbf{Event sliding window.}
Conversation is produced by walking an event sliding window of a fixed
size $W$ over $\mathcal{T}$ with a pointer $p_k$ that advances one event
per round. At round $k$, the window covers the $W$ most recent events
ending at the leading event $e_{p_k}$. The trailing events let the user
simulator issue an \emph{optional follow-up query} that revisits earlier
context, while the leading event $e_{p_k}$ supplies the current
motivated query over its freshly attached images $\mathcal{I}_k$. Visual
context is delivered cumulatively, so the assistant at round $k$ sees
$\bigcup_{j\le k}\mathcal{I}_j$.

\noindent \textbf{Cross-round memory.}
To carry memory across the long horizon, the round state is summarized
rather than replayed verbatim. After round $k$ we emit a faithful
brief summary $\sigma_k$ of the exchange and update a
running memory by structured append so that the user simulator 
for the next round is conditioned on the
accumulated memory rather than the raw transcript,
\begin{equation}
\small
  r_{k+1} \sim \pi_{\text{user}}
    \bigl(\,\cdot \mid \mathcal{W}_{k+1},\ S_k,\ \mathcal{P}\,\bigr).
\end{equation}
The round stream is finally partitioned into sessions
$\mathcal{D} = (D_1, \dots, D_L)$, each a coherent multi-turn
conversation, so that a single $(\mathcal{P},\mathcal{C},\mathcal{F})$
triple yields a complete multi-session dataset.

% \noindent \textbf{Quality Control.} Synthesized dialogue is verified by two-stage
% inspection. A per-chunk audit scans fixed-size windows of rounds
% for persona violations, core-event drift, hallucinations, and internal
% contradictions; a cross-chunk audit then catches contradictions that
% span chunk boundaries and severed continuous event.
% Every flagged round is rewritten by a repair pass that conditions
% on a local window of neighboring rounds to preserve continuity.
% In the timeline stage, an additional expert inspection checks
% whether the dialogue stays faithful to the persona and follows the
% core event through.

% =====================================================================
\subsection{Evaluation Framework}
\label{sec:eval-framework}

\noindent \textbf{Typed question bank.}
From the finalized dataset $\mathcal{D}$ we synthesize a typed
question bank $\mathcal{Q}$ by sampling a context window of rounds and
prompting an LLM to emit items. Each item is a tuple
\begin{equation}
\small
  q = (x,\, A,\, \mathcal{F}_q,\, \tau),
  \qquad A = (a_0, a_1, \dots, a_m),
\end{equation}
where $x$ is the question text, $A$ is an ordered answer list whose
head $a_0$ is the gold and whose tail entries are progressively
coarser alternatives used for graded scoring, $\mathcal{F}_q$ is the
set of supporting-fact round identifiers, and $\tau$ is the type. We
organize the eight types along the three capabilities of
\emph{memorizing}, \emph{reasoning}, and \emph{interpreting}.
\emph{Memorizing} types probe whether evidence is faithfully retained
and located: single-session retrieval (\textsc{SS}) grounds the answer in
one session, file management (\textsc{FM}) asks which image matches a
description, and factual judgment (\textsc{FJ}) is a four-option
multiple-choice item with distractors.
\emph{Reasoning} types require fusing or transforming evidence:
multi-session reasoning (\textsc{MS}) draws facts from $\ge\!2$
sessions ($|\{\,\mathrm{sess}(f) : f\in\mathcal{F}_q\}| \ge 2$),
multimodal reasoning (\textsc{MR}) reads a value visible in an image
or PDF page but absent from the text, and temporal reasoning
(\textsc{TR}) resolves dates, ordering, or time spans over
$\mathcal{T}$.
\emph{Interpreting} types target unstated meaning: implicit inference
(\textsc{II}) composes $\ge\!2$ clues into an answer never stated
outright, and thematic reasoning (\textsc{TH}) bundles the
decisions of one case thread into a structured answer. Per-type
descriptions, sampling strategies, and prompts are given in
Appendix~\ref{sec:appendix-examples}.

% \noindent \textbf{Quality Control.}
% Each generated question undergoes a validation pass that enforces both
% well-formedness and evidence consistency. The central constraint is
% that a question may only cite evidence the model was actually shown:
% supporting facts that fall outside the sampled context window are
% filtered out, and any question left without valid support is discarded.
% Malformed questions are re-prompted once and otherwise removed.
% This procedure guarantees that every retained question is answerable
% from the evidence it cites. Details in Appendix~\ref{sec:appendix-examples}.

% =====================================================================

